SurgPub-Video: A Comprehensive Surgical Video Dataset for Enhanced Surgical Intelligence in Vision-Language Model

Vision-Language Models (VLMs) have shown significant potential in surgical scene analysis, yet existing models are limited by frame-level datasets and lack high-quality video data with procedural surgical knowledge. To address these challenges, we make the following contributions: (i) SurgPub-Video, a comprehensive dataset of over 3,000 surgical videos and 25 million annotated frames across 11 specialties, sourced from peer-reviewed clinical journals, (ii) SurgLLaVA-Video, a specialized VLM for surgical video understanding, built upon the TinyLLaVA-Video architecture that supports both video-level and frame-level inputs, and (iii) a video-level surgical Visual Question Answering (VQA) benchmark, covering diverse 11 surgical specialities, such as vascular, cardiology, and thoracic. Extensive experiments, conducted on the proposed benchmark and three additional surgical downstream tasks (action recognition, skill assessment, and triplet recognition), show that SurgLLaVA-Video significantly outperforms both general-purpose and surgical-specific VLMs with only three billion parameters. The dataset, model, and benchmark will be released to enable further advancements in surgical video understanding.

==> tex/3_method_old.tex <==
\section{SurgPub-Video Dataset}
\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{fig/framework.pdf}
\caption{The construction of the SurgPub-Video Benchmark}
\label{framework}
\end{figure*}


\subsection{Pipeline Overview}
We propose a fully automated, agent-orchestrated pipeline to construct SurgPub-Video dataset.
Our pipeline integrates multiple AI agents to sequentially preprocess surgical videos, extract textual and visual contents, and generate structured VQA pairs.
First, surgical videos from peer-reviewed journals undergo automated speech recognition (ASR) to obtain accurate transcripts with sentence-level timestamps.
Second, a multimodal AI agent comprehensively analyzes textual and visual contents, extracting surgical entities, actions, and their semantic relationships.
Third, another AI agent automatically formulates multiple-choice and open-ended questions grounded on identified surgical concepts and authoritative narration evidence.
Finally, medical experts validate and refine the automatically generated questions and answers, ensuring clinical accuracy and semantic consistency across modalities.

\subsection{Video Preprocessing and Text Extraction}
In Stage 1, we preprocess raw surgical videos by extracting medically accurate textual narrations and segmenting videos into meaningful clips.
We employ the OpenAI Whisper model for automatic speech recognition, providing robust sentence-level transcription of narration from surgical video contents.
To further ensure the medical accuracy of the transcripts, we introduce a GPT-4o-based agent for secondary correction of domain-specific terminologies.
This correction leverages structured surgical reports as authoritative references, significantly improving the accuracy of specialized medical terms and abbreviations.
Subsequently, we utilize an AI agent guided by GPT-4o to intelligently segment the videos based on transcript semantics and surgical event boundaries.
% This adaptive segmentation strategy avoids arbitrary truncation of key surgical actions, producing coherent video clips of approximately 15 to 30 seconds.


\subsection{Multimodal Content Understanding and Concept Extraction
}
Stage 2 involves comprehensive multimodal understanding, employing an AI agent to extract structured surgical entities and their semantic relationships.
We build a unified GPT-4o-driven multimodal analysis framework, which simultaneously processes both textual transcripts and corresponding video frames effectively.
This AI agent identifies critical surgical entities, including anatomical structures, pathological lesions, surgical instruments, procedural steps, and operative actions.
The extracted entities are subsequently mapped onto a standardized surgical ontology to normalize synonyms, abbreviations, and terminological variations across sources.
The AI agent further establishes semantic relations between identified entities, specifically instrument-action associations and anatomical structure-pathology correlations.
Finally, automated filtering based on content richness scores ensures retention of high-quality clips containing sufficient clinical relevance and surgical details for analysis.

\subsection{Automated VQA Pair Generation}
In Stage 3, an AI agent automatically generates high-quality surgical question-answer pairs, forming the core content of SurgPub-Video.
We employ large language model-driven question generation strategies, explicitly targeting diverse question categories including instrument usage, procedural goals, and anatomical relationships.
To enhance clinical relevance, we design reasoning-based questions derived explicitly from causal explanations and rationales articulated within video narrations.
This approach ensures generated questions possess authoritative clinical grounding, covering prediction of surgical outcomes, operative rationale, and risk-related decision-making processes.
For answer generation, the AI agent produces both open-ended responses and multiple-choice questions with intentionally crafted distractors to reduce guessability.
% All generated answers maintain medical accuracy, conciseness, and precise alignment with textual evidence, facilitating robust learning outcomes from the dataset.

\subsection{Refinement and Quality Control}
Stage 4 implements rigorous human expert reviews to refine automatically generated VQA pairs, ensuring medical correctness and semantic consistency.
Medical imaging specialists and experienced surgeons jointly examine each question-answer pair, verifying clinical accuracy and explicit alignment with corresponding videos.
The expert team systematically evaluates generated prompts and questions, identifying potential biases or inaccuracies introduced during the AI-driven generation process.
Quality metrics, including acceptance rate, revision frequency, and rejection proportions, are recorded comprehensively to monitor overall dataset reliability and validity.
Expert-identified issues inform iterative improvements, allowing continuous updates to AI agents' question generation prompts, concept extraction processes, and filtering criteria.
This iterative human-in-the-loop approach significantly elevates data quality, ultimately establishing SurgPub-Video as an authoritative, clinically accurate resource for surgical VQA research.










\section{SurgLLaVA-Video Model }

SurgLLaVA-Video is a multimodal large language model specifically optimized for surgical video question answering (VQA) tasks. 
%
Its core architecture is derived from TinyLLaVA-Video and enhanced through fine-tuning on SurgPub-Video. 
%
\paragraph{Vision Encoder}
The primary component of the model is the vision encoder $\mathbf{V}_{\phi}$. 
%
This encoder is responsible for extracting critical visual features from raw surgical video frames $X_t\in \mathbb{R}^{H \times W \times 3}$, where $H$ and $W$ represent the height and width of the frame, respectively. Specifically, for each frame in the video, its corresponding feature representation $H_t$ is obtained as follows:
\begin{equation}  
H_t = \mathbf{V}_{\phi}(X_t).
\end{equation}  
This process ensures that fine-grained visual information, such as the movement of surgical instruments, the identification of anatomical structures, and the sequence of complex procedures, is effectively captured from surgical videos, laying the groundwork for subsequent understanding tasks.

\paragraph{Connector}
Secondly, the connector $\mathbf{P}_{\theta}$ plays a crucial role in SurgLLaVA-Video, as it is responsible for effectively linking the sequence of frame-level visual features extracted by the vision encoder with the language model. For the sequence of visual features $\left\{H_1, H_2, \ldots, H_N\right\}$ obtained from the surgical video, the connector processes them using a cross-attention mechanism to generate a unified and semantically rich visual embedding sequence $E_V$. This process aims to bridge the heterogeneity between the visual and linguistic modalities, ensuring that visual information can be correctly parsed by the language model. Its operation can be represented as:
\begin{equation}  
E_V = \mathbf{P}_{\theta}(\text{Concat}(H_1, \ldots, H_N)).
\end{equation}
Through this mechanism, the model is able to integrate the temporal dynamics and spatial details of surgical videos and transform this complex visual information into a format understandable by the language model, thereby supporting high-level semantic reasoning.

\paragraph{Large Language Model}

Finally, the small language model $\mathbf{F}_{\psi}$ constitutes the core understanding and response generation module of SurgLLaVA-Video. It combines the visual embeddings $E_V$ generated by the connector with user-posed surgical-related text questions $Q$. The language model performs joint reasoning on these multimodal inputs and generates a corresponding textual answer $A$. This process can be summarized as:
\begin{equation}
    A = \mathbf{F}_{\psi}(Q, E_V)
\end{equation}

To enhance the model's efficiency and adapt to the prolonged nature of surgical videos, SurgLLaVA-Video incorporates video-level group resampling. This technique involves intelligently selecting a representative subset of frames from the entire video sequence, rather than processing every single frame. This strategy ensures that the most informative frames are retained while redundant ones are discarded, thereby reducing computational overhead without significant loss of critical information.


By fine-tuning on SurgPub-Video, SurgLLaVA-Video is capable of understanding complex medical scenarios, identifying key events during surgery, and providing accurate, professional answers to questions related to surgical instruments, operational steps, or abnormal conditions. This integrated architecture makes SurgLLaVA-Video a powerful tool for surgical video analysis and interactive question answering.


==> tex/AAAI26_Checklist.tex <==
\section*{Reproducibility Checklist}
\newcommand{\answerYes}{\textbf{yes}}
\newcommand{\answerNO}{\textbf{no}}
\newcommand{\answerNA}{\textbf{NA}}

Unless specified otherwise, please answer ''yes'' to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

\subsection*{This paper:}

\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)\\
    Answer: \answerYes{}
    \item Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper (yes/no)\\
    Answer: \answerYes{}
\end{itemize}

\subsection*{Does this paper make theoretical contributions? (yes/no) If yes, please complete the list below.}
Answer: \answerYes{}


\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)\\
    Answer: \answerYes{}
    \item Proofs of all novel claims are included. (yes/partial/no)\\
    Answer: \answerYes{}
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)\\
    Answer: \answerYes{}
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)\\
    Answer: \answerYes{}
\end{itemize}

\subsection*{Does this paper rely on one or more datasets? (yes/no)}
Answer: \answerYes{}

\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)\\
    Answer: \answerNA{}
    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)\\
        Answer: \answerNA{}
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (yes/no/NA)\\
    Answer: \answerYes{}
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisfying. (yes/partial/no/NA)\\
    Answer: \answerNA{}
\end{itemize}

\subsection*{Does this paper include computational experiments? (yes/no)}
Answer: \answerYes{}

\begin{itemize}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)\\
    Answer: \answerYes{}
    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)\\
        Answer: \answerYes{}
    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)\\
    Answer: \answerYes{}
    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)\\
    Answer: \answerYes{}
    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)\\
        Answer: \answerYes{}
    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)\\
    Answer: \answerYes{}
    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)\\
    Answer: \answerYes{}
    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)\\
        Answer: \answerYes{}
    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)\\
    Answer: \answerYes{}
    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. (yes/partial/no/NA)\\
    Answer: \answerYes{}
\end{itemize}
